Joint Seat Allocation 2018: An algorithmic perspective

Until 2014, admissions to the Indian Institutes of Technology (IITs) were conducted under one umbrella, whereas the admissions to the non-IIT Centrally Funded Government Institutes (CFTIs) were conducted under a different umbrella, the Central Seat Allocation Board. In 2015, a new Multi-Round Multi-Run Deferred Acceptance joint seat allocation process was implemented, improving the efficiency and productivity of concerned stakeholders. The process brings all CFTIs under one umbrella for admissions: 100 institutes and approximately 39000 seats in 2018. In this scheme, each candidate submits a single choice list over all available programs, and receives no more than a single seat from the system, based on the choices and the ranks in the relevant merit lists. Significantly, overbooking of seats is forbidden. In this report, we provide details of our safe, fair and optimal algorithm. Novel features include the ability to handle multiple merit lists, seat guarantee across multiple rounds, implementing reservation, and de-reservation rules, handling escalation of ranks due to a revision of marks by state boards during the allocation process, and dealing with last minute de-recognition of other backward caste categories. A notable rule required the allocation of supernumerary seats to females, provided the program did not have a sufficient desired percentage, while, at the same time, not reducing the number of seats available to non-females. Looking forward, we posit first that it is inevitable that different colleges will prefer different mechanisms of judging merit, and assigning relative rank. We believe the ability of our algorithm to gracefully handle multiple merit lists gives us hope to express optimism that all undergraduate admissions in the country, beyond the CFTIs, can beneficially use the suggested scheme.

==> mincutoff.tex <==
\section{Computing \mc\ }%and setting \cc\ }
\label{sec:mincutoff}


%For computing \mc\ for a virtual program $p$ for round $i+1$, we proceed as follows. If there was any vacancy in virtual program $p$ in 
%the allotment of round $i$, we assign $\mc(p)$ as $\infty$. Otherwise, we compute set $S(p)$
%of candidates allocated to $p$ in the seat allocation of round $i$ and proceed as follows. From $S(p)$, we remove the following
%candidates
%\begin{enumerate}
%\item Those who rejected or withdrew
%\item Those whose seat got canceled
%\end{enumerate} 
%$\mc(p)$ is defined as the rank of the worst rank candidate in the resulting $S(p)$. If $S(p)$ is empty, we define $\mc(p)$ as 0.
%
\noindent {\bf Computing \mc: } The word minimum in
min-cut-off is used to indicate that in future rounds, the cutoff (or
closing rank) can actually become worse (i.e., larger) than the
min-cut-off.  Consider any virtual program $p$. We use the output $\wl(p)$ of $i$th round to compute $\mc(p)$ for
$(i+1)$th round as follows.  First note that it is entirely possible
that $p$ may have unfilled seats. These unfilled seats, may or
may not be de-reserved. 
%In the sequel, we assume that merit lists have been updated based on marks revision. 
We temporarily construct a \emph{reduced} waitlist for 
   $p$ by removing the following kinds of candidates:
     \begin{enumerate}
      \item Those who opted for reject or withdraw.
%      \item Those who were awarded a seat through the Defense Services
%        Priority Allocation (DS) (these candidates should be
%        considered for min-cut-off of the DS virtual program and not
%        for other virtual programs)
%      \item Those with CatChange=1
%      \item Those with CatChange=4
%      \item If $p$ is an engineering program then those with a
%        decrease in the marks in the engineering exam. Conversely, if
%        $p$ is an architecture program then those with decrease in
%        subjects related to the architecture program.
     \item Those whose seat got cancelled because they suffered CatChange=1 or CatChange=4 at the reporting center in the previous round. 
     \end{enumerate}

     \noindent
     We then set $\mc(p)$ for the next round as follows:
     \begin {itemize}

\item   If the reduced waitlist is non-empty, $\mc(p)$ is set to
   $\rank(y,p)$, where $y$ is the last candidate in the reduced wait
   list. Note again that, $\rank$ here stores the extended merit list rank
     after revision. \footnote{Recall Definition \ref{def:primary_merit_list}.
     {\bf Example}: If $p$ is an OBC-NCL virtual program then we use
     the last rank in the standard OBC-NCL merit list. On the other
     hand if $p$ is an SC virtual program then we use the last rank in
     the extended merit list, which, to recall is constructed by
     taking the SC rank list
     followed by the PC-SC rank list.}
     
\item     If the reduced waitlist is empty, $\mc(p)$ is set to 0. Thus, nobody applying to $p$ in the next round will get any min-cut-off benefit.
\end{itemize}


%\begin{center}
%  \begin{figure}[h!]
%    \includegraphics[height=0.9\textheight]{Figures/MC-benefit-and-computation-final-version}
%    %\includegraphics[width=0.9\textwidth]{Figures/MC-benefit-and-computation-final-version}
%    \caption{Setting and maintaining \cc\ flag across rounds}
%    \label{Figure:Setting-CatChange}
%  \end{figure}
%\end{center}
%
%\noindent {\bf Setting} \mc: Candidates who are to be penalized (the so-called \cc\ penalty) have
%their \cc\ flag set to 1. They are also added to the $\cc$
%list. Candidates whose seats were cancelled, but are not to be
%penalized still need to have their credentials updated.  In the mining
%example of Section~\ref{subsec:changes_to_other_DA}, the candidate
%should not get the same mining seat.  This situation is recorded by
%setting their \cc\ flag to 4. (By default, recall that the \cc\ flag
%is 2.) Further, it is set to 3 if a candidate's credentials change,
%but the seat doesn't get cancelled.\footnote{A candidate with \cc\ set
%  to 1 candidate cannot get the freeze assurance even in future rounds
%  with the way ``freeze'' is implemented (see
%  Section~\ref{subsec:multiround_virtualprefs})}.
%Figure~\ref{Figure:Setting-CatChange} depicts how the \cc\ flag
%is set in various situations.
%
%\noindent {\bf Computing \mc: } While the notion of \mc\ is very candidate
%friendly, there are complications due to the intertwined change in
%credentials, and the change in the merit order. The word minimum in
%min-cut-off is used to indicate that in future rounds, the cutoff (or
%closing rank) can actually become worse (i.e., larger) than the
%min-cut-off.  We consider the output $\wl(p)$, and set $\mc(p)$ for
%the next round as follows.  First note that it is entirely possible
%that programs may have unfilled seats. These unfilled seats, may or
%may not be de-reserved.  In the sequel, we assume that merit lists
%have been updated based on marks revision. We temporarily construct a \emph{reduced} waitlist for a
%   virtual program $p$ by removing the following kinds of candidates:
%     \begin{enumerate}
%      \item Those who opted for reject
%      \item Those who were awarded a seat through the Defense Services
%        Priority Allocation (DS) (these candidates should be
%        considered for min-cut-off of the DS virtual program and not
%        for other virtual programs)
%      \item Those with CatChange=1
%      \item Those with CatChange=4
%      \item If $p$ is an engineering program then those with a
%        decrease in the marks in the engineering exam. Conversely, if
%        $p$ is an architecture program then those with decrease in
%        subjects related to the architecture program.
%     \end{enumerate}
%
%     We then set $\mc(p)$ for the next round as follows:
%     \begin {itemize}
%
%\item   If the reduced waitlist is non-empty, $\mc(p)$ is set to
%   $\rank(y,p)$, where $y$ is the last candidate in the reduced wait
%   list. Note again that, $\rank$ here stores the extended merit list rank
%     after revision. \footnote{Recall Definition \ref{def:primary_merit_list}.
%     {\bf Example}: If $p$ is an OBC-NCL virtual program then we use
%     the last rank in the standard OBC-NCL merit list. On the other
%     hand if $p$ is an SC virtual program then we use the last rank in
%     the extended merit list, which, to recall is constructed by
%     taking the SC rank list
%     followed by the PC-SC rank list.}
%     
%\item     If the reduced waitlist is empty, $\mc(p)$ is set to 0. Thus, nobody applying to $p$ in the next round will get any min-cut-off benefit.
%\end{itemize}
%
%   Table~\ref{figure:MC-benefit-and-computation} states the conditions
%   under which a candidate can be considered for \mc\ benefit as well
%   as the computation of \mc.
%
%
%\begin{table}
%\begin{tabular}{|p{3.5cm}|l|p{3.5cm}|p{3.5cm}|}
%\hline
%
%MarksChange & CatChange value & Min-cut-off benefit  & Consideration for Min-cut-off computation  \\
%({\footnotesize{consider ENG if the allotted program is ENG, consider ARC if allotted program is ARC}}) & & ({\footnotesize{If given, a supernumerary seat may be created for a candidate if his/her rank is better than min-cut-off}}) & ({\footnotesize{"considered" implies that the candidate will be  included in the reduced waitlist}}) \\ \hline
%I/U & 1 & Not given & Not considered \\ \hline
%I/U & 2 & Given & considered \\ \hline
%I/U & 3 & Given & considered \\ \hline
%I/U & 4 & Given & Not considered \\ \hline
%D & 1 & Not given & Not considered \\ \hline
%D & 2 & Given & Not considered \\ \hline
%D & 3 & Given & Not considered \\ \hline
%D & 4 & Given & Not considered \\ \hline
%\end{tabular}
%\caption{The conditions under which a candidate is considered for $\mc(p)$ computation and $\mc(p)$ benefits for a virtual program.}
%\label{figure:MC-benefit-and-computation}
%\end{table}
%
%
%
%   %Effectively, we are preparing to satisfy, e.g., the freeze
%          %assurance.
%%      \begin{itemize}
%%      \item the last CML rank for an OP virtual program
%%      \item last OBC for OBC
%%      \item last PC-SC rank for SC
%%      \item last PC-ST for ST
%%      \item last PC-CML-PwD for OP-PD
%%      \item last PC-OBC-PD for OBC-PD
%%      \item last PC-SC-PwD for SC-PD,
%%      \item last PC-ST-PwD for ST-PD.
%%      \end{itemize}
%


==> ties.tex <==
{\color{red}
\section{DA with multiple candidates having same rank}
\label{sec:DAwithTies}

Suppose multiple candidates obtain exactly the same rank. In the
situation when we are forced to reject some candidate due to the
possibility that the program is oversubscribed, we have to also reject
(and remove) all other candidates in the waiting list who
also have the same rank.  This may not be always possible.

We modify lines \ref{line:apply_noties}-\ref{line:apply_endnoties} of
Algorithm~\ref{alg:DA} as stated in Algorithm \ref{alg:DAwithTies} to
allow such candidates to obtain seats in the program on a
supernumerary basis. We keep $\wl(p)$ fully ordered at each step, by
choosing an arbitrary order between candidates in $\wl(p)$ who have
the exact same rank as per $\merit(p)$.  

There are two concepts involved here.  First, when an attempt is made
to remove a candidate $x$, a removal of all candidates with the same
rank of $x$ may cause the waitlist which is initially overflowing, to
now underflow.  To identify this situation, we compute the length $G$ of
the waitlist, and the length $L$ of the list of candidates all of whom
have the same rank as $x$.  If the difference between the two exceeds
or matches the capacity, we are free to remove all such
candidates. Second, if this condition is not satisfied, it is not
possible to remove all candidates with rank of $x$.  However, there
might be candidates $w \in \cc$ who also have the same rank.  The
algorithm checks if it is all right to remove only this subset.
}
{\color{red}
\begin{algorithm}[h]
\label{alg:DAwithTies}
\caption{DeferredAcceptanceWithTies} 
Same INPUT and OUTPUT as in Algorithm \ref{alg:DA}
\begin{algorithmic}[1]
\LineComment Everything before Line~\ref{line:apply_noties} in Algorithm~\ref{alg:DA}
\Function{RemoveAndReject}{w,p}
  \State $G \gets |\wl(p)|$
  \State $L \gets \mbox{number of people with rank same as w}$
  \Comment L is at least 1
  \State $L_1 \gets \mbox{number of people with rank same as w and such
people in \cc}$
  \If{$(G - L) \geq c(p)$}
    \State Remove all people with rank(w)
    \State \Call{Reject}{} all people with rank(w)
  \Else \Comment Removing such people may cause p to be under capacity
    \If{$(G - L_1) \geq c(p)$}
      \State Remove all people corresponding to $L_1$ 
      \State Call Reject on all people corresponding to $L_1$
    \EndIf
  \EndIf
\EndFunction

\Function{PenaltyRemoveAndReject}{w,p}
  \State $G \gets |\wl(p)|$
  \State $L_1 \gets \mbox{number of people with rank same as w and such
people in \cc}$
  \If{$(G - L_1) \geq c(p)$}
      \State Remove all people corresponding to $L_1$ 
      \State Call Reject on all people corresponding to $L_1$
  \EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

The algorithm also considers the case when we want to remove only
candidates who belong to category change.  This can happen when such
candidates clear the \mc\ but because we are not allowed to have
supernumerary seats; they need to be out of the waitlist.

We remark in passing that there is a certain simplicity, and thus
beauty,  in processing candidates in any order.  When multiple
candidates have the same rank, this poses a challenge.  The proposed algorithm
%Algorithm~\ref{alg:DAwithTies}, 
responds to this challenge in an
elegant fashion.}
